Novel Joint Estimation and Decoding Metrics for Short-Block length Transmission Systems

This paper presents Bit-Interleaved Coded Modulation metrics for joint estimation detection using training or reference signal transmission strategies for short to long block length channels. We show that it is possible to enhance the performance and sensitivity through joint detection-estimation compared to standard receivers, especially when the channel state information is unknown and the density of the training dimensions is low. The performance analysis makes use of a full 5G transmitter and receiver chains for both Polar and LDPC coded transmissions paired with BPSK/QPSK modulation schemes. We consider transmissions where reference signals are interleaved with data and both are transmitted over a small number of OFDM symbols so that near-perfect channel estimation cannot be achieved. This is particularly adapted to mini-slot transmissions for ultra-reliable, low-latency communications (URLLC) or for short packet random access use cases. We characterize the performance for up to eight receiving antennas in order to determine the performance gain offered by the proposed BICM detection in realistic base station receiver scenarios. Our findings demonstrate that when the detection windows used in the metric units is on the order of four modulated symbols the proposed BICM metrics can be used to achieve detection performance that is close to that of a coherent receiver with perfect channel state information for both polar and LDPC coded configurations. Furthermore, we show that for transmissions with low DMRS density, a good trade-off can be achieved in terms of additional coding gain and improved channel estimation quality by adaptive DMRS power adjustment.

==> figures/mimo/chain_tx.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,544); %set diagram left start at 0, and has height of 544

%Shape: Rectangle [id:dp880256749655464]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (148,335) -- (171.84,335) -- (171.84,412.2) -- (148,412.2) -- cycle ;
%Shape: Rectangle [id:dp36775314886186916]
\draw  [fill={rgb, 255:red, 228; green, 74; blue, 198 }  ,fill opacity=1 ] (213,335) -- (245.7,335) -- (245.7,412.2) -- (213,412.2) -- cycle ;
%Shape: Rectangle [id:dp6756309667052469]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (363,337) -- (386.84,337) -- (386.84,414.2) -- (363,414.2) -- cycle ;
%Straight Lines [id:da26720768988872434]
\draw    (172.41,342.5) -- (209.41,342.5) ;
\draw [shift={(212.41,342.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da9482237606287145]
\draw [line width=0.75]    (173.41,367.5) -- (210.41,367.5) ;
\draw [shift={(213.41,367.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da9739424261790588]
\draw    (172.41,403.5) -- (208.84,403.55) ;
\draw [shift={(211.84,403.55)}, rotate = 180.08] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da8575489855555561]
\draw    (277.28,342.71) -- (360.11,343.84) ;
\draw [shift={(363.11,343.88)}, rotate = 180.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da6611549737622966]
\draw    (278.28,367.71) -- (363.11,367.88) ;
\draw [shift={(366.11,367.88)}, rotate = 180.11] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da02648169621152663]
\draw    (277.28,402.71) -- (363.11,402.88) ;
\draw [shift={(366.11,402.88)}, rotate = 180.11] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da8427573503515995]
\draw    (283,326.67) -- (282.96,335.62) ;
\draw [shift={(282.95,338.62)}, rotate = 270.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da43464009560523453]
\draw    (283.07,352.58) -- (283.07,361.58) ;
\draw [shift={(283.07,364.58)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da8909523967505615]
\draw    (284,381.67) -- (284,394.67) ;
\draw [shift={(284,397.67)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da05187200041726081]
\draw    (245.33,343) -- (274.28,342.74) ;
\draw [shift={(277.28,342.71)}, rotate = 179.48] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da4535895823153351]
\draw    (244.33,368) -- (275.28,367.74) ;
\draw [shift={(278.28,367.71)}, rotate = 179.51] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da27959790891816183]
\draw    (243.33,403) -- (274.28,402.74) ;
\draw [shift={(277.28,402.71)}, rotate = 179.51] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da6478672041508438]
\draw    (120.31,371.93) -- (138.56,371.97) -- (147,371.99) ;
\draw [shift={(150,372)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da6253574318476358]
\draw    (333.52,343.87) -- (333,456) ;
%Straight Lines [id:da2585785358415096]
\draw    (340,368) -- (339,448) ;
%Straight Lines [id:da964703843568244]
\draw    (345,344) -- (344.11,442.88) ;
%Shape: Rectangle [id:dp9034490230498529]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (351.11,432.88) -- (390,432.88) -- (390,461) -- (351.11,461) -- cycle ;
%Straight Lines [id:da8111130341654331]
\draw    (344.11,442.88) -- (350.89,442.75) ;
%Straight Lines [id:da3301203991894407]
\draw    (352,448) -- (339,448) ;
%Straight Lines [id:da4062120423332719]
\draw    (333,456) -- (353,456) ;
%Straight Lines [id:da6700546205264183]
\draw    (377.77,431) -- (377.77,418) ;
\draw [shift={(377.77,415)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da7623828107653625]
\draw    (388,373) -- (410,373) ;
\draw [shift={(413,373)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Shape: Rectangle [id:dp17317676221142586]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (50.11,289.88) -- (90.31,289.88) -- (90.31,310.93) -- (50.11,310.93) -- cycle ;
%Shape: Rectangle [id:dp6159921138835014]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (119,290.93) -- (171.31,290.93) -- (171.31,310.67) -- (119,310.67) -- cycle ;
%Shape: Rectangle [id:dp34451369681722877]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (187.11,289.93) -- (233.63,289.93) -- (233.63,310.52) -- (187.11,310.52) -- cycle ;
%Shape: Rectangle [id:dp8466085345225443]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (250.11,289.93) -- (290.31,289.93) -- (290.31,309.93) -- (250.11,309.93) -- cycle ;
%Shape: Rectangle [id:dp6419952190293643]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (310.11,290.93) -- (350.31,290.93) -- (350.31,310.93) -- (310.11,310.93) -- cycle ;
%Shape: Rectangle [id:dp9300516554466642]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (369.11,290.93) -- (403.16,290.93) -- (403.16,310) -- (369.11,310) -- cycle ;
%Shape: Rectangle [id:dp2237976981754557]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (421.11,290.93) -- (471.33,290.93) -- (471.33,310.33) -- (421.11,310.33) -- cycle ;
%Straight Lines [id:da5461794617341896]
\draw    (22.31,301.93) -- (40.56,301.97) -- (49,301.99) ;
\draw [shift={(52,302)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da39386899741063797]
\draw    (90.31,300.93) -- (108.56,300.97) -- (117,300.99) ;
\draw [shift={(120,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da43858013105006244]
\draw    (169.33,301) -- (178.56,300.97) -- (187,300.99) ;
\draw [shift={(190,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da330099392114779]
\draw    (233.33,301) -- (240.56,300.97) -- (249,300.99) ;
\draw [shift={(252,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da27869113541421175]
\draw    (291.33,301) -- (298.56,300.97) -- (307,300.99) ;
\draw [shift={(310,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da8465814925282863]
\draw    (350.33,301) -- (357.56,300.97) -- (366,300.99) ;
\draw [shift={(369,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da7968750577220802]
\draw    (412.56,300.97) -- (402.16,301) -- (421,301) ;
\draw [shift={(424,301)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Straight Lines [id:da5666814102001669]
\draw    (473.31,300.93) -- (491.56,300.97) -- (500,300.99) ;
\draw [shift={(503,301)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
%Shape: Rectangle [id:dp08839107838888072]
\draw  [fill={rgb, 255:red, 74; green, 190; blue, 228 }  ,fill opacity=1 ] (429.11,320.93) -- (463.16,320.93) -- (463.16,340) -- (429.11,340) -- cycle ;
%Straight Lines [id:da6062487459708867]
\draw    (444.83,321.9) -- (444.83,313.9) ;
\draw [shift={(444.83,310.9)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;

% Text Node
\draw (407,288.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$N_{d}$};
% Text Node
\draw (163.5,351.5) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-90] [align=left] {Transmitter};
% Text Node
\draw (376.5,361.5) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-90] [align=left] {Receiver};
% Text Node
\draw (213,366) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Channel };
% Text Node
\draw (223,380.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{H}$};
% Text Node
\draw (273.41,332.9) node [anchor=north west][inner sep=0.75pt]    {$\oplus $};
% Text Node
\draw (273.41,357.9) node [anchor=north west][inner sep=0.75pt]    {$\oplus $};
% Text Node
\draw (273.41,391.9) node [anchor=north west][inner sep=0.75pt]    {$\oplus $};
% Text Node
\draw (175,330.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$x_{1}$};
% Text Node
\draw (175,355.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$x_{2}$};
% Text Node
\draw (175,386.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$x_{_{ \begin{array}{l}
N_{_{T}}\\
\end{array}}}$};
% Text Node
\draw (175.41,370.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\vdots $};
% Text Node
\draw (317.41,376.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\vdots $};
% Text Node
\draw (288,323.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$z_{1}$};
% Text Node
\draw (288,347.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$z_{2}$};
% Text Node
\draw (286,385.07) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$z_{_{ \begin{array}{l}
N_{R}\\
\end{array}}}$};
% Text Node
\draw (317,329.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$y_{1}$};
% Text Node
\draw (317,354.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$y_{2}$};
% Text Node
\draw (315,386.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$y_{_{ \begin{array}{l}
N_{R}\\
\end{array}}}$};
% Text Node
\draw (353.11,435.88) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Channel \\Estimator};
% Text Node
\draw (54.99,297.62) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-359.66] [align=left] {\begin{minipage}[lt]{22.57pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize CRC \ Attach.}
\end{center}

\end{minipage}};
% Text Node
\draw (120.02,298.92) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-359.66] [align=left] {\begin{minipage}[lt]{36.36pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize CB \ Seg. \& CB crc att.}
\end{center}

\end{minipage}};
% Text Node
\draw (189.13,292.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{30.52pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Channel Encoding}
\end{center}

\end{minipage}};
% Text Node
\draw (257.13,293.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{21.06pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Rate Match.}
\end{center}

\end{minipage}};
% Text Node
\draw (317.13,294.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{20.3pt}\setlength\topsep{0pt}
\begin{center}
{\tiny CB \ concat.}
\end{center}

\end{minipage}};
% Text Node
\draw (423.13,293.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{32.2pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Resource \ Mapping}
\end{center}

\end{minipage}};
% Text Node
\draw (376.13,294.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{19.36pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Modulation}
\end{center}

\end{minipage}};
% Text Node
\draw (23,292.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$A\ bits$};
% Text Node
\draw (60,280.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$B=A+CRC$};
% Text Node
\draw (199.13,275.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{8.78pt}\setlength\topsep{0pt}
\begin{center}
{\tiny intlv}
\end{center}

\end{minipage}};
% Text Node
\draw (243.13,276.92) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-359.66] [align=left] {\begin{minipage}[lt]{40.46pt}\setlength\topsep{0pt}
\begin{center}
{\tiny Sublk ntlv, bit select, intlv}
\end{center}

\end{minipage}};
% Text Node
\draw (432.13,326.92) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-359.66] [align=left] {\begin{minipage}[lt]{21.31pt}\setlength\topsep{0pt}
\begin{center}
{\tiny dmrs insertion}
\end{center}

\end{minipage}};
% Text Node
\draw (478,288.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$N_{d} +N_{P}$};
% Text Node
\draw (482,307.4) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$x_{N}$};


\end{tikzpicture}


==> figures/plot/mimo/ldpc_mimo2x2.tex <==
% % Preamble:
%  \pgfplotsset{width=7cm,compat=newest} \pgfplotsset{every axis/.append style={
%     font=\footnotesize,
%     thin,
%     tick style={ultra thin}}}
% \begin{tikzpicture}[scale=0.5]
%     \begin{loglogaxis}[
%         xlabel=\textsc{Dof},
%         ylabel=$L_2$ Error
%     ]
%     %  see above for this macro:
%     \plotcoords
%     \legend{$d=2$,$d=3$,$d=4$,$d=5$,$d=6$}
%     \end{loglogaxis}
% \end{tikzpicture}

% \begin{tikzpicture}
%         \begin{semilogyaxis}[xlabel=SNR (dB),
%       ,ylabel=BLER, xmin=0,xmax=20, ymin=1e-5,ymax=1]
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}



%legend pos=outer north east
%legend pos=north west
%legend pos=north east

      \begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER, xmin=-5,xmax=25, ymin=0.0005,ymax=0.5, legend pos=north east,
            grid=both,
            ]

\addplot+[smooth,teal, mark options={scale=1, fill=teal},mark=*] coordinates {
%(6	, 0.141643059490085)
(7	, 0.0920810313075506)
%(8	, 0.0770416024653313)
%(9	, 0.0623441396508728)
%(10, 	0.0467726847521048)
(11, 	0.0262329485834208)
%(12, 	0.0194174757281553)
%(13, 	0.0137023842148534)
%(14, 	0.00801603206412826)
(15, 	0.00648004147226542)
%(16, 	0.00411878578195148)
%(17, 	0.00270219147728808)
%(18, 	0.00189175384498969)
(19, 	0.00124584200231727)
%(20, 	0.00076)
};
\addlegendentry{Perfect CSI, BILCM, $(2\times2)$}


%%%%%%%%%%%%% % N=1

\addplot+[smooth, densely dotted, black, mark options={ scale=1, fill=black},mark=*] coordinates {
%(8	, 0.136986301369863)
(9	, 0.0965250965250965)
%(10, 	0.0789889415481833)
%(11, 	0.060790273556231)
%(12, 	0.0496277915632754)
(13, 	0.0251382604323781)
%(14, 	0.0176709666018731)
%(15, 	0.0122579063495955)
%(16, 	0.00780335544284042)
(17, 	0.00642095800693463)
%(18, 	0.00406388426057626)
%(19, 	0.00292500292500292)
%(20, 	0.00189803742929811)
(21, 	0.00126752351256116)
%(22, 	0.00078)
};
\addlegendentry{No CSI, BILCM, $(2\times2)$, N=1}


\addplot+[smooth, dashed, magenta, mark options={scale=1, fill=magenta},mark=*] coordinates {
%(7	, 0.120336943441637)
(8	, 0.0843170320404722)
%(9	, 0.0677048070412999)
%(10, 	0.0577700751010976)
%(11, 	0.034494653328734)
(12, 	0.0229832222477591)
%(13, 	0.017415534656914)
%(14, 	0.0114902907043548)
(15, 	0.00816393174953057)
%(16, 	0.00521947909598622)
%(17, 	0.00351506204084502)
%(18, 	0.00230776331579433)
%(19, 	0.00177377299253242)
(20, 	0.00120697146719452)
};
\addlegendentry{No CSI, BILCM, $(2\times2)$ N=4}


%%%%%%%%%%%%%%%%%%%4 rx


\addplot+[smooth,teal, mark options={scale=1, fill=teal},mark=oplus] coordinates {
(-2, 	0.134048257372654)
%(-1, 	0.0735835172921266)
(0	, 0.0543183052688756)
%(1	, 0.0347101700798334)
(2	, 0.0199760287654814)
%(3	, 0.0105596620908131)
(4	, 0.00543951261966928)
%(5	, 0.00216314434662225)
(6	, 0.00143213129779738)
(7	, 0.00084)
%(8	, 0.00036)
%(9	, 0.0001)
};
  \addlegendentry{Perfect CSI, BILCM, $(4\times4)$}


\addplot+[smooth, densely dotted, gray, mark options={ scale=1, fill=gray, solid},mark=oplus] coordinates {
(5	, 0.108108108108108)
%(6	, 0.089126559714795)
(7	, 0.0493096646942801)
%(8	, 0.0266666666666667)
(9	, 0.0193836014731537)
%(10, 	0.01170138076293)
(11, 	0.00553311569744923)
%(12, 	0.00289762684361508)
(13, 	0.00177856825255669)
(14, 	0.0008)
};
\addlegendentry{No CSI, BILCM, $(4\times4)$, N=1}


\addplot+[smooth, dashed, violet, mark options={scale=1, fill=violet, solid},mark=oplus] coordinates {
% -1	0.94521)
%(0,	0.82479)
%(-1,	0.45045045045045)
(2	, 0.107411385606874)
%(3	, 0.0706214689265537)
(4	, 0.0386996904024768)
%(5	, 0.0233426704014939)
(6	, 0.0145158949049209)
%(7	, 0.0076657723265619)
(8	, 0.00329283150581185)
%(9	, 0.00217907650737617)
(10, 	0.00100927523945055)
%(11, 	0.00054)
%(12, 	0.00017)

};
\addlegendentry{No CSI,  BILCM, $(4\times4)$, N=4}


%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}


==> figures/plot/mimo/polar_mimo2x2.tex <==
% % Preamble:
%  \pgfplotsset{width=7cm,compat=newest} \pgfplotsset{every axis/.append style={
%     font=\footnotesize,
%     thin,
%     tick style={ultra thin}}}
% \begin{tikzpicture}[scale=0.5]
%     \begin{loglogaxis}[
%         xlabel=\textsc{Dof},
%         ylabel=$L_2$ Error
%     ]
%     %  see above for this macro:
%     \plotcoords
%     \legend{$d=2$,$d=3$,$d=4$,$d=5$,$d=6$}
%     \end{loglogaxis}
% \end{tikzpicture}

% \begin{tikzpicture}
%         \begin{semilogyaxis}[xlabel=SNR (dB),
%       ,ylabel=BLER, xmin=0,xmax=20, ymin=1e-5,ymax=1]
\pgfplotsset{
    tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    legend style={nodes={scale=0.7, transform shape}, font=\tiny, legend cell align=left},
    every axis/.append style={line width=0.5pt}
}


%legend pos=outer north east
%legend pos=north west
%legend pos=north east

      \begin{tikzpicture}
              \begin{semilogyaxis}[xlabel=SNR (dB),
            ,ylabel=BLER, xmin=-5,xmax=25, ymin=0.0005,ymax=0.5, legend pos=north east,
            grid=both, xminorgrids,
            yminorgrids,
            minor grid style={solid}
            ]




\addplot+[smooth,teal, mark options={scale=1, fill=teal},mark=*] coordinates {
(3	,0.107296137339056)
%(4	,0.0646412411118294)
%(5	,0.0411861614497529)
(6	,0.0282805429864253)
%(7	,0.025025025025025)
%(8	,0.0158654608916389)
(9	,0.00815195239259803)
%(10,	0.0057540710052362)
%(11,	0.00477076475359)
(12,	0.00257738601510348)
%(13,	0.00156452899854499)
%(14,	0.00113356835983994)
(15,	0.00063)
% (16,	0.00042)
% (17,	0.00021)
% (18,	0.00014)
        };
        \addlegendentry{Perfect CSI, BIPCM, $(2\times2)$}


%%%%%%%%%%%%% % N=1

\addplot+[smooth, densely dotted, black, mark options={ scale=1, fill=black},mark=*] coordinates {
(6	,0.0969932104752667)
% (7	,0.0846023688663283)
% (8	,0.0476417341591234)
(9,	0.0384319754035357)
% (10,	0.0271444082519001)
% (11,	0.0191828122002686)
(12,	0.0129684865776164)
% (13,	0.00667334000667334)
% (14,	0.00542269941977116)
(15,	0.00348650721706994)
% (16,	0.00245152116888529)
% (17,	0.00127538006325885)
(18,	0.00088)
% (19,	0.00049)
% (20,	0.00031)
% (21,	0.00018)
% (22,	0.00015)
};
\addlegendentry{No CSI, BIPCM, $(2\times2)$, N=1}


\addplot+[smooth, dashed, magenta, mark options={scale=1, fill=magenta},mark=*] coordinates {
(4	,0.108225108225108)
% (5	,0.0755857898715042)
% (6	,0.0506842372022301)
(7	,0.0381533765738268)
% (8,	0.024770869457518)
% (9	,0.015956598053295)
(10,	0.0102239034863511)
% (11,	0.00557880055788006)
% (12,	0.00518726008922087)
(13,	0.00304497426996742)
% (14,	0.00194450385984016)
% (15,	0.00115009948360533)
(16,	0.00064)
% (17,	0.00051)
% (18,	0.00023)
% (19,	0.00019)
% (20,	0.0001)
};
\addlegendentry{No CSI, BIPCM, $(2\times2)$, N=4}


%%%%%%%%%%%%%%%%%%%4 rx


\addplot+[smooth,teal, mark options={scale=1, fill=teal},mark=oplus] coordinates {

(-3,	0.0889679715302491)
%(-2,	0.0571102227298686)
(-1,	0.0258665287118469)
%(0	,0.0150647785477553)
(1	,0.00984155102844208)
%(2	,0.00441715623481603)
(3	,0.00238123586141207)
(4	,0.00094)
% (5	,0.00053)
% (6	,0.00028)
        };
  \addlegendentry{Perfect CSI, BIPCM, $(4\times4)$}


\addplot+[smooth, densely dotted, gray, mark options={ scale=1, fill=gray, solid},mark=oplus] coordinates {
(5	,0.0824402308326463)
%(6	,0.0580383052814858)
(7	,0.0314564328405159)
%(8	,0.018618506795755)
(9	,0.0132065504490227)
%(10,	0.00679624847084409)
(11,	0.0036330608537693)
%(12,	0.00196730341720604)
(13,	0.00109698438991213)
% (14,	0.00076)
% (15,	0.00058)
};
\addlegendentry{No CSI, BIPCM, $(4\times4)$, N=1}


\addplot+[smooth, dashed, violet, mark options={scale=1, fill=violet, solid},mark=oplus] coordinates {
(1	,0.113378684807256)
%(2	,0.0633713561470216)
(3	,0.0354609929078014)
%(4	,0.0186950831931202)
(5	,0.0118736642127761)
%(6	,0.00761672633102293)
(7	,0.00295168098231943)
%(8	,0.00153959847271832)
(9	,0.00076)
%(10,	0.00046)
% (11,	0.00017)
% (12,	0.00011)
};
\addlegendentry{No CSI, BIPCM, $(4\times4)$, N=4}


%%%%%%%
        \end{semilogyaxis}
    \end{tikzpicture}

